Exploring the Potential of Large Language Models in Generating Code-Tracing Questions for Introductory Programming Courses

In this paper, we explore the application of large language models (LLMs) for generating code-tracing questions in introductory programming courses. We designed targeted prompts for GPT4, guiding it to generate code-tracing questions based on code snippets and descriptions. We established a set of human evaluation metrics to assess the quality of questions produced by the model compared to those created by human experts. Our analysis provides insights into the capabilities and potential of LLMs in generating diverse code-tracing questions. Additionally, we present a unique dataset of human and LLM-generated tracing questions, serving as a valuable resource for both the education and NLP research communities. This work contributes to the ongoing dialogue on the potential uses of LLMs in educational settings.

==> paper_notes.tex <==
\section{Paper Notes}
\cite{10.1145/3501385.3543957} uses OpenAI CodeX to generate coding exercise and code explanations, but education is not just about giving explanation but to ask questions to help student understand their code. 

\cite{10.1145/3456565.3460054,10.1145/3498343.3498347,noble2022automated} described an application of automatic generating tracing questions in a tracing table format, rather than in natural language. This limits its methodology in a conventional program analysis and template-based question generation, but cannot deal with open-ended natural language tracing question. 


\cite{narayanan2023enhancing} use ChatGPT3.5 to generate counterfactual questions in natual language, but they did not systematically evaluate the quality and helpfulness comparing with human-write questions. 

\cite{10.1145/3159450.3159608}

\cite{hassan2023students} showed that tracing can help students solve EiPE (Explain in Plain English) questions in coding classes, and thus, help them understand the codes' execution behaviors. They also noticed that students may fail to trace code in 3 ways: 1) they did not consider tracing, 2) they traced incorrectly because of the misunderstanding of the concepts, and 3) they did not choose good inputs that exposed the purposes of the code.


\cite{russell-etal-2022-bu} built an application called Trace Generator to generate automatically graded code tracing questions so it provided comprehensive and understandable feedback for students to learn from their mistakes. They also discussed the importance of code comprehension skills in programming.


\cite{stankov2023smart} The authors argued that code tracing tasks can provide a good insight into the level of basic knowledge and understanding of the underlying programming language and some basic programming concepts in general. However, maintaining complexity consistency when designing questions that contain code snippets for students' tests can be challenging, especially when working with large classes of students. To address this issue, the authors propose the use of CodeCPP, a tool that automatically generates code-tracing questions by modifying certain parts of a given initial template program code to generate different code snippets and questions. The complexity of each generated code snippet is calculated and depending on its value, the code variation is either saved or discarded. 


\ran{TODO: important}
\cite{hassan2021exploring} The authors propose a method called "Reverse Tracing," which means students need to figure out the input based on the value of an output. This method is designed to help instructors identify the misconceptions that led students to write incorrect code. The authors argue that this approach is more effective than traditional methods because it focuses on the students' thought processes and the errors they make, rather than simply identifying the correct solution.
(Analysis: GPT-4 can also generate reverse tracing questions, but almost all human-created tracing questions are regular tracing questions.)

\aysa{Background. Tracing is useful.}
\cite{sekiya2013tracing} created a tracing quiz set with various Ruby codes and administered it to five student groups. They identified seven common misconceptions from the students' responses, with "Neglect For Loop" (NFL) being the most significant. Over half of the errors were explained by these misconceptions, and students with the NFL misconception performed notably worse. The authors recommend early detection of these misconceptions to improve programming skills.


